Memory-Aware Denial-of-Service Attacks on Shared Cache in Multicore Real-Time Systems

In this paper, we identify that memory performance plays a crucial role in the feasibility and effectiveness for performing denial-of-service attacks on shared cache. Based on this insight, we introduce new cache DoS attacks, which can be mounted from the user-space and can cause extreme worst-case execution time (WCET) impacts to cross-core victims -- even if the shared cache is partitioned -- by taking advantage of the platform's memory address mapping information and HugePage support. We deploy these enhanced attacks on two popular embedded out-of-order multicore platforms using both synthetic and real-world benchmarks. The proposed DoS attacks achieve up to 111X WCET increases on the tested platforms.

==> acknowledgement.tex <==
\section*{Acknowledgements} \label{acknowledge}
This research is supported in part by NSF CNS 1718880, CNS 1815959, NSA
Science of Security initiative contract \#H98230-18-D-0009, and 
a gift from the Ripple University Blockchain Research Initiative.

==> memory.tex <==
\section{Impact of Memory Performance to Cache DoS
  Attacks}\label{sec:memory}

In this section, we provide an experimental evidence on the impact of
memory performance to 
%motivating example to show how memory performance  affects
the effectiveness of cache DoS attacks.

%As discussed in Section~\ref{sec:background}, 
Cache DoS
attacks~\cite{valsan2016taming,bechtel2019dos} attempt to exhaust
internal hardware buffers of a shared non-blocking cache to induce
cache blocking. The cache becomes unblocked when the cache internal
buffers become available again, which would require accesses to main
memory. Therefore, we hypothesize that if the access to memory takes
longer, the longer the cache would be blocked. 
In other words, poor memory performance would increase the
effectiveness of cache DoS attacks.

To test the hypothesis,
%impact of memory performance on the efficacy of DoS attacks,
we perform the same cache DoS attack experiments as
in~\cite{bechtel2019dos}. That is, we measure the slowdown of a
synthetic victim task on Core 0 while co-scheduling cache DoS attackers
on Cores 1-3 on a Raspberry Pi 3 platform; the LLC is partitioned so that 
the attackers can't directly affect the victim's performance through
cache evictions; the victim's working-set size fits in its given LLC 
while the attackers do not (i.e. their working set size is greater than the size of the LLC). 

Unlike previous experiments, however, we make use of the Raspberry Pi 3's
ability manually control the memory frequency and transfer rate of its LPDDR2 memory
module by modifying the \textit{sdram\_freq} parameter in the 
\texttt{config.txt} file in the boot partition. By default, the Pi 3
operates at 450Mhz (900 MT/s, as DDR transfers both rising and falling edges). 
In our testing, we configure the memory to run from 1000
MT/s down to 100 MT/s, in increments of 100 MT/s. 
%Note that such system changes
%would not be realistically feasible for attackers as memory frequency control
%is usually reserved for users with privileged access or completely unavailable. 
%Instead, with these tests we hope to evaluate whether memory performance
%can impact the effectiveness of cache DoS attacks.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.40\textwidth]{figs/perf_vs_memfreq}
  \caption{ Effect of memory frequency on performance slowdown caused due to 
  cache DoS attacks. }
  \label{fig:perf-vs-memfreq}
\end{figure}

Figure~\ref{fig:perf-vs-memfreq} shows the results. As we expected, the
operating transfer rate of the shared memory, and by proxy the memory's
performance, has significant impact to the effectiveness of cache DoS
attacks. As we decrease the transfer rate, the slowdown experienced by the
victim task significantly increases. In particular, when we lower the
frequency to only 100 MT/s, we observe more than \emph{900X WCET
  increase} of the victim task. 

The results confirm our hypothesis that memory performance is a crucial
factor to the effectiveness of cache DoS attacks and that slow memory
performance ``improves'' the effectiveness of cache DoS attacks.

%% Note that the victim was \emph{not} supposed to be affected by slow
%% DRAM performance as its working-set fit in its own cache partition.
%% The reason for this "unexpected" massive WCET increase of the victim
%% is that the slow DRAM access speed results in longer shared cache blocking
%% when the attackers generate lots of concurrent cache misses even
%% though the attackers are on different cores and accessing their own 
%% dedicated cache partitions.

%% Based on this finding, we hypothesize that DoS attacks can be more
%% effective if they target main memory, in addition to the shared LLC,
%% with the goal of decreasing its performance.
%% To achieve this, we make use
%% of a system's memory address mapping information and HugePage support as we
%% detail in the following section.

%% \iffalse
The simplest and most straight-forward way to improve the effectiveness
of cache DoS attacks is to directly control the performance
of the main memory system, for example, by changing the memory bus frequency as we did in this experiment.
%In addition to altering frequency, this could also be done by lowering
%the total number of DRAM banks (e.g. remove DIMM sticks, use
%single-rank DRAM, etc.). This is because fewer banks would lead to an
%increased possibility for bank contention to occur and would also lead
%to increased memory access times~\cite{yun2015ecrts}. 
However, it either requires root privilege do to so or not supported at all. For example, Raspberry Pi 3, which we uses in this experiment, does support memory clock speed changes via a configuration file for the bootloader, but only the root can change the file. On the other hand, Raspberry Pi 4, which we use in later part of the paper, does not allow memory frequency change even for the root user.
According to our threat model, attackers would neither have the required
privileges nor physical access to the target machine in order for such
approaches to be viable. 

In this work, we focus on software approaches to create more effective DoS attacks by generating \emph{memory access patterns} that
are slower to process at the hardware level, and thereby improve the
effectiveness of cache DoS attacks.
%% Specifically, As a result, we believe that such improvements to DoS attacks can only be realized
%% through software modifications that enable the attacks to cause bank contention,
%% as frequency control wouldn't be possible.
To achieve this, we make use
of a system's memory address mapping information and HugePage support as we
detail in the following section.
%% \fi

%%% %% 
%% Cache DoS attacks have been shown to work on both in-order and
%% out-of-order core architectures~\cite{valsan2016taming,bechtel2019dos}.
%% Specifically, both previous works used sequential access pattern-based
%% attacks (see Section~\ref{sec:seqattack}), that sought to exhaust
%% internal cache hardware structures by repeatedly accessing a large 1D
%% array.  While effective, sequential memory access patterns 
%% %we believe a notable downside to these attacks is
%% can be efficiently handled in memory such patterns would exploit DRAM
%% bank level parallelism and locality in DRAM row-buffer. 
%% %% . That is, all attack
%% %% instances can be mapped to different memory banks and be processed in
%% %% parallel. Furthermore, sequential arrays can also be mapped to the
%% %% same row within a bank which allows for better memory access times and
%% %% overall system performance as it reduces the need for  memory to
%% %% switch between rows (i.e. fewer precharges and activations would be
%% %% required).

%% This improvement in system operation can be undesirable from a cache DoS attack 
%% point-of-view. Since their goal is to induce cache blocking by exhausting internal
%% hardware structures in shared cache, reduced memory access times could improve
%% the rate at which structure entries are freed. Based on this relation, we theorize 
%% that memory performance could also impact shared cache DoS attacks as it could 
%% directly influence the duration which cache spends blocked.


==> simulation.tex <==
\section{Hardware Simulation}~\label{sec:simulation}

\begin{figure*}[htp]
  \centering
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/firesim_bc_bwread}
    \caption{ BwRead victim. }
    \label{fig:firesim-bc-bwread}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/firesim_bc_lmlp}
    \caption{ LatencyRead victim. }
    \label{fig:firesim-bc-lmlp}
  \end{subfigure}
  \caption{Impacts of cache DoS attacks on BwRead victims run on medium
  BOOM cores. The attackers and victim run on their own dedicated cores.}
  \label{fig:firesim-bc}
\end{figure*}

In this section, we attempt to recreate our real-world findings for the Odroid XU4
on a cycle-accurate full system simulator. We use the FPGA-acclerated
FireSim simulator~\cite{karandikar2018firesim} as it provides improved accuracy 
faster simulation speed compared to other full-system simulators. In FireSim,
we employ the RISC-V BOOM~\cite{celio2015berkeley} out-of-order core configuration
as its designed to resemble out-of-order ARM cores like the Cortex-A15. In our 
setup, we simulate a quad-core processor comprised of medium BOOM cores and 
configure them to emulate the Cortex-A15's cache parameters as much as possible. 
Specifically, we set the local and global MLPs of the cores to match the A15 by increasing 
the number of MSHRs in the L1D and L2 caches to 6 and 11, respectively. 
The full system parameters can be seen in Figure~\ref{tbl:firesim-setup}. For
the OS, we employ the mainline RISC-V port of Linux kernel version 4.15.

\begin{table}[h]
  \centering
  \begin{adjustbox}{width=.45\textwidth}
  \begin{tabular}{|c|c|}
    \hline
    \multirow{2}{*}{Processor}  & Quad-core BOOM (RISC-V ISA), 2.13 GHz \\
								& out-of-order, 2-wide, 4-issue, ROB: 64, LSQ: 16/16 \\ \hline
    \multirow{2}{*}{Caches}		& L1-I/D: 32/32KiB, 4(I)/2(D) way, MSHRs: 1(I)/6(D)\\ 
								& LLC: 512 KiB, 16-way, 11 MSHRs, 64-byte lines \\ \hline
    System Bus      			& TileLink, out-of-order completion, round-robin \\ \hline
    DRAM Controller 			& FR-FCFS, open-page policy, scheduler window: 8 \\ \hline
    DRAM  						& DDR3-2133, 1 rank, 8 banks, 32 KiB row-buffers \\ \hline
  \end{tabular}
  \end{adjustbox}
  \caption{FireSim system configuration.}
  \label{tbl:firesim-setup}
\end{table}

We run the same synthetic victim experiments in our FireSim setup as we did on
the embedded platforms from Section~\ref{sec:eval-synthetic}. That is, we run
the victim task alone on Core 0 and co-schedule an increasing number of attacker
tasks on Cores 1-3 while measuring the victim's average response time.

The results can be seen in Figure~\ref{fig:firesim-bc}. Like the Odroid XU4,
we find that our BankRead and BankWrite attackers have the most impact to both 
victim tasks with the write version incurring a higher slowdown. Unlike the XU4,
we find that the simulation only requires two BankRead/Write attackers to cause
significant slowdown with a third attacker providing effectively negligible 
additional impact.


